Invariant Filtering for Legged Humanoid Locomotion on Dynamic Rigid Surfaces

State estimation for legged locomotion over a dynamic rigid surface (DRS), which is a rigid surface moving in the world frame (e.g., ships, aircraft, and trains), remains an under-explored problem. This paper introduces an invariant extended Kalman filter that estimates the robot's pose and velocity during DRS locomotion by using common sensors of legged robots (e.g., inertial measurement units (IMU), joint encoders, and RDB-D camera). A key feature of the filter lies in that it explicitly addresses the nonstationary surface-foot contact point and the hybrid robot behaviors. Another key feature is that, in the absence of IMU biases, the filter satisfies the attractive group affine and invariant observation conditions, and is thus provably convergent for the deterministic continuous phases. The observability analysis is performed to reveal the effects of DRS movement on the state observability, and the convergence property of the hybrid, deterministic filter system is examined for the observable state variables. Experiments of a Digit humanoid robot walking on a pitching treadmill validate the effectiveness of the proposed filter under large estimation errors and moderate DRS movement. The video of the experiments can be found at: https://youtu.be/ScQIBFUSKzo.

==> excess.tex <==
% , we first explicitly consider the data inaccuracies associated with the contact frame orientation {\small$\small \mathbf{R}^c_{t}$} and the surface frame orientation {\small ${\mathbf{R}}_{t} \mathbf{h}_R(\mathbf{q}_t)$}.}
% in Eq.~\eqref{equ: position measuremment}.}

% \YanMod{[[[[[To address the inaccurate knowledge of the surface orientation, we assume that the true orientation is corrupted by uncertainty {\small$\mathbf{w}^{DRS}_{t}$} as:}
% % the uncertainty of treadmill orientation. Thus, we have
% % The true orientation of the surface is corrupted by the uncertainty of treadmill orientation. Thus, we have
% \YanMod{[[[explain tn, or just use t.]]]}
% \vspace{-0.05in}
% \begin{equation}
% \small
% \begin{aligned}
%      {\mathbf{R}}^{DRS}_{t_n}
%     =
%     \text{exp}(- \mathbf{w}^{DRS}_{t_n}) {\mathbf{\tilde{R}}}^{DRS}_{t_n}
%     \approx
%     (\mathbf{I}_3 -{(\mathbf{w}^{DRS}_{t_n})_\times)}  \tilde{\mathbf{R}}^{DRS}_{t_n},
% \end{aligned}
%     \label{eqn: surface pose uncertainty}
%     \vspace{-0.05in}
% \end{equation}
% where
% {\small
% $
% \mathbf{\tilde{R}}^{DRS}_{t_n}$} is the \YanMod{inaccurately known DRS orientation}
% and {\small$\mathbf{w}^{DRS}_{t_n}$} is the white Gaussian zero-mean inaccuracy expressed in the world frame.
% \YanMod{]]]]]}

%%%%%%%%%%%%%%%
% \YanMod{[[[[[}
% \YanMod{To handle the inaccuracy of the encoder reading $\tilde{\mathbf{q}}_{t}$},
% the support-foot orientation
% % {\small ${\mathbf{R}}^{c}_{t}$}
% {\small $\mathbf{R}_{t_n}  \mathbf{h}_R(\mathbf{q}_{t_n})$}
% is
% expressed and approximated as:
% % Let the forward kinematics {\small$\mathbf{h}_R(\mathbf{q}) \in SO(3)$} be the support-foot orientation in the robot base (see Fig.\ref{Fig: overview}), and denote {\small$\mathbf{h}_R = [\mathbf{h}_{R,1},~\mathbf{h}_{R,2},~\mathbf{h}_{R,3}] $}.
% % Then the support-foot orientation in the world, , can be 
% \vspace{-0.05in}
% \begin{equation}
% \small
% \label{equ: decompose wRf}
% \begin{aligned}
%     % \mathbf{R}^c_{t_n}
%     % &= 
%     \mathbf{R}_{t_n}  \mathbf{h}_R(\mathbf{q}_{t_n})
%     % =\mathbf{R}_{t_n} \mathbf{h}_R(\mathbf{\tilde{q}}_{t_n}-\mathbf{w}^q_{t_n})
%     \approx
%     \mathbf{R}_{t_n}\mathbf{h}_R(\mathbf{\tilde{q}}_{t_n})-\mathbf{R}_{t_n}\mathbf{J}_{h_R}(\tilde{\mathbf{q}}_{t_n},\mathbf{w}^q_{t_n}).
% \end{aligned}
% \vspace{-0.05in}
% \end{equation}
% Here the matrix
% {\small$\small \mathbf{J}_{h_R}(\tilde{\mathbf{q}}_{t_n},\mathbf{w}^q_{t_n})$} is obtained by computing the Jacobian of each column of
% % {\small$\mathbf{h}_R$},
% ;
% that is:
% \vspace{-0.05 in}
% \begin{equation}
% \small
%      \mathbf{J}_{h_R}
%     \triangleq
%     \begin{bmatrix}
%         \frac{\partial \mathbf{h}_{R,1}}{\partial {\mathbf{q}}_{t}} (\tilde{\mathbf{q}}_{t_n}) \mathbf{w}^q_{t_n},~
%         \frac{\partial \mathbf{h}_{R,2}}{\partial {\mathbf{q}}_{t}}
%         (\tilde{\mathbf{q}}_{t_n})
%         \mathbf{w}^q_{t_n},~
%         \frac{\partial \mathbf{h}_{R,3}}{\partial {\mathbf{q}}_{t}}
%         (\tilde{\mathbf{q}}_{t_n})
%         \mathbf{w}^q_{t_n}
%     \end{bmatrix},
% \vspace{-0.05 in}
% \label{equ: JhR}
% \end{equation}
% where {\small$[\mathbf{h}_{R,1},~\mathbf{h}_{R,2},~\mathbf{h}_{R,3}]:=\mathbf{h}_R$.}
% \YanMod{]]]]]}


% Substituting Eqs.~\eqref{eqn: surface pose uncertainty}-\eqref{equ: JhR} into Eq.~\eqref{equ: alligned normal vector} yields:
% \vspace{-0.05 in}
% \begin{equation}
% \small
% \label{equ:haha}
% \begin{aligned}
% &\mathbf{R}_{t_n}^T \mathbf{\tilde{R}}^{DRS}_{t_n}
% \begin{bmatrix}
%     0
%     ~
%     0
%     ~
%     1
% \end{bmatrix}^T
% +
% \mathbf{R}^T_{t_n}(-\mathbf{w}^{DRS}_{t_n})_\times \mathbf{\tilde{R}}^{DRS}_{t_n}
% \begin{bmatrix}
%     0
%     ~
%     0
%     ~
%     1
% \end{bmatrix}^T
% \\
% \approx &
% \mathbf{h}_R(\mathbf{\tilde{q}}_{t_n})
% {\begin{bmatrix}
%     0
%     ~
%     0
%     ~
%     1
% \end{bmatrix}^T}
% -
% \tfrac{\partial \mathbf{h}_{R,3}}{\partial \tilde{\mathbf{q}}_{t_n}}(\tilde{\mathbf{q}}_{t_n})
% \mathbf{w}^q_{t_n},
% \end{aligned}
% \vspace{-0.05 in}
% \end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%
